Personalized Federated Learning via Sequential Layer Expansion in Representation Learning

Federated learning ensures the privacy of clients by conducting distributed training on individual client devices and sharing only the model weights with a central server. However, in real-world scenarios, the heterogeneity of data among clients necessitates appropriate personalization methods. In this paper, we aim to address this heterogeneity using a form of parameter decoupling known as representation learning. Representation learning divides deep learning models into 'base' and 'head' components. The base component, capturing common features across all clients, is shared with the server, while the head component, capturing unique features specific to individual clients, remains local. We propose a new representation learning-based approach that suggests decoupling the entire deep learning model into more densely divided parts with the application of suitable scheduling methods, which can benefit not only data heterogeneity but also class heterogeneity. In this paper, we compare and analyze two layer scheduling approaches, namely forward (\textit{Vanilla}) and backward (\textit{Anti}), in the context of data and class heterogeneity among clients. Our experimental results show that the proposed algorithm, when compared to existing personalized federated learning algorithms, achieves increased accuracy, especially under challenging conditions, while reducing computation costs.

==> reference.tex <==
@article{jacobs1963fine,
  title={Fine particles, thin films and exchange anisotropy (effects of finite dimensions and interfaces on the basic properties of ferromagnets)},
  author={Jacobs, IS and Bean, CP},
  journal={Spin arrangements and crystal structure, domains, and micromagnetics},
  volume={3},
  pages={271--350},
  year={1963}
}

@article{mactaggert2019california,
  title={The California privacy rights and enforcement act of 2020},
  author={Mactaggert, A},
  journal={Retrieved October},
  volume={21},
  number={2020},
  pages={19--0019},
  year={2019}
}

% Federated Leanring
@inproceedings{mcmahan2017communication,
  title={Communication-efficient learning of deep networks from decentralized data},
  author={McMahan, Brendan and Moore, Eider and Ramage, Daniel and Hampson, Seth and y Arcas, Blaise Aguera},
  booktitle={Artificial intelligence and statistics},
  pages={1273--1282},
  year={2017},
  organization={PMLR}
}

%PFL servey
@article{tan2022towards,
  title={Towards personalized federated learning},
  author={Tan, Alysa Ziying and Yu, Han and Cui, Lizhen and Yang, Qiang},
  journal={IEEE Transactions on Neural Networks and Learning Systems},
  year={2022},
  publisher={IEEE}
}

% FedProx
@article{li2020federated,
  title={Federated optimization in heterogeneous networks},
  author={Li, Tian and Sahu, Anit Kumar and Zaheer, Manzil and Sanjabi, Maziar and Talwalkar, Ameet and Smith, Virginia},
  journal={Proceedings of Machine learning and systems},
  volume={2},
  pages={429--450},
  year={2020}
}

% SCAFFLOD
@inproceedings{karimireddy2020scaffold,
  title={Scaffold: Stochastic controlled averaging for federated learning},
  author={Karimireddy, Sai Praneeth and Kale, Satyen and Mohri, Mehryar and Reddi, Sashank and Stich, Sebastian and Suresh, Ananda Theertha},
  booktitle={International conference on machine learning},
  pages={5132--5143},
  year={2020},
  organization={PMLR}
}

%Meta Learning
%MAML
@inproceedings{finn2017model,
  title={Model-agnostic meta-learning for fast adaptation of deep networks},
  author={Finn, Chelsea and Abbeel, Pieter and Levine, Sergey},
  booktitle={International conference on machine learning},
  pages={1126--1135},
  year={2017},
  organization={PMLR}
}

%Reptile
@article{nichol2018first,
  title={On first-order meta-learning algorithms},
  author={Nichol, Alex and Achiam, Joshua and Schulman, John},
  journal={arXiv preprint arXiv:1803.02999},
  year={2018}
}

% transfer learning
@article{li2019fedmd,
  title={Fedmd: Heterogenous federated learning via model distillation},
  author={Li, Daliang and Wang, Junpu},
  journal={arXiv preprint arXiv:1910.03581},
  year={2019}
}

@article{chen2020fedhealth,
  title={Fedhealth: A federated transfer learning framework for wearable healthcare},
  author={Chen, Yiqiang and Qin, Xin and Wang, Jindong and Yu, Chaohui and Gao, Wen},
  journal={IEEE Intelligent Systems},
  volume={35},
  number={4},
  pages={83--93},
  year={2020},
  publisher={IEEE}
}

% Reperesentation Learning
% FedPer
@article{arivazhagan2019federated,
  title={Federated learning with personalization layers},
  author={Arivazhagan, Manoj Ghuhan and Aggarwal, Vinay and Singh, Aaditya Kumar and Choudhary, Sunav},
  journal={arXiv preprint arXiv:1912.00818},
  year={2019}
}

%multi-task learning
@article{smith2017federated,
  title={Federated multi-task learning},
  author={Smith, Virginia and Chiang, Chao-Kai and Sanjabi, Maziar and Talwalkar, Ameet S},
  journal={Advances in neural information processing systems},
  volume={30},
  year={2017}
}

%LG
@article{liang2020think,
  title={Think locally, act globally: Federated learning with local and global representations},
  author={Liang, Paul Pu and Liu, Terrance and Ziyin, Liu and Allen, Nicholas B and Auerbach, Randy P and Brent, David and Salakhutdinov, Ruslan and Morency, Louis-Philippe},
  journal={arXiv preprint arXiv:2001.01523},
  year={2020}
}

%FedRep
@inproceedings{collins2021exploiting,
  title={Exploiting shared representations for personalized federated learning},
  author={Collins, Liam and Hassani, Hamed and Mokhtari, Aryan and Shakkottai, Sanjay},
  booktitle={International conference on machine learning},
  pages={2089--2099},
  year={2021},
  organization={PMLR}
}

% FedROD
@article{chen2021bridging,
  title={On bridging generic and personalized federated learning for image classification},
  author={Chen, Hong-You and Chao, Wei-Lun},
  journal={arXiv preprint arXiv:2107.00778},
  year={2021}
}

% FedBABU
@article{oh2021fedbabu,
  title={Fedbabu: Towards enhanced representation for federated image classification},
  author={Oh, Jaehoon and Kim, Sangmook and Yun, Se-Young},
  journal={arXiv preprint arXiv:2106.06042},
  year={2021}
}

% FedCP
@inproceedings{zhang2023fedcp,
  title={Fedcp: Separating feature information for personalized federated learning via conditional policy},
  author={Zhang, Jianqing and Hua, Yang and Wang, Hao and Song, Tao and Xue, Zhengui and Ma, Ruhui and Guan, Haibing},
  booktitle={Proceedings of the 29th ACM SIGKDD Conference on Knowledge Discovery and Data Mining},
  pages={3249--3261},
  year={2023}
}

% curriculum in FL
@inproceedings{vahidian2023curricula,
  title={When do curricula work in federated learning?},
  author={Vahidian, Saeed and Kadaveru, Sreevatsank and Baek, Woonjoon and Wang, Weijia and Kungurtsev, Vyacheslav and Chen, Chen and Shah, Mubarak and Lin, Bill},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={5084--5094},
  year={2023}
}

@inproceedings{bengio2009curriculum,
  title={Curriculum learning},
  author={Bengio, Yoshua and Louradour, J{\'e}r{\^o}me and Collobert, Ronan and Weston, Jason},
  booktitle={Proceedings of the 26th annual international conference on machine learning},
  pages={41--48},
  year={2009}
}
